Concurrent Transmission for Multi-Robot Coordination

An efficient communication mechanism forms the backbone for any multi-robot system to achieve fruitful collaboration and coordination. Limitation in the existing asynchronous transmission based strategies in fast dissemination and aggregation compels the designers to prune down such requirements as much as possible. This also restricts the possible application areas of mobile multi-robot systems. In this work, we introduce concurrent transmission based strategy as an alternative. Despite the commonly found difficulties in concurrent transmission such as microsecond level time synchronization, hardware heterogeneity, etc., we demonstrate how it can be exploited for multi-robot systems. We propose a split architecture where the two major activities - communication and computation are carried out independently and coordinate through periodic interactions. The proposed split architecture is applied on a custom build full networked control system consisting of five two-wheel differential drive mobile robots having heterogeneous architecture. We use the proposed design in a leader-follower setting for coordinated dynamic speed variation as well as the independent formation of various shapes. Experiments show a centimeter-level spatial and millisecond-level temporal accuracy while spending very low radio duty-cycling over multi-hop communication under a wide testing area.

==> 2-background.tex <==
\section{Background}\label{sec:back}

In a networked multi-robot system, every robot is considered to be an independent unit. Fig.~\ref{fig:layer}(a) shows a simplified diagram depicting the main hardware and software modules of one such unit. In the software part, there are three key entities -- \textit{Operating System}, \textit{Control System}, and at least one application, termed as \textit{MRC Application}. In a multi-robot setting, the \textit{Network Stack} partially overlapping with the Operating System plays the key role of handling the communication among the participating robots.
% commcommunication Currently used mechanisms for multi-robot communication mostly uses asynchronous transmission where a node can decide to transmit independently. Synchronous transmission based strategies, gradually are gaining more attention. In this work we propose to use the same under a multi-robot platform as detailed below.

\begin{figure}[t!]
\begin{center}
\includegraphics[width=\linewidth]{Figures/layer.pdf}
\end{center}
\caption{Part (a) shows the general modules of an independent networked robotic system. Part (b) shows the separation of the \textit{Network Unit} and \textit{Computing \& Control Unit}. Part (c) shows a network among multiple independent robotic systems.} \label{fig:separation}
\end{figure}

\subsection{Asynchronous and concurrent transmission based communication}

Systematic access to the shared medium is a common and fundamental issue when more than a pair of devices try to communicate with each other. The \textit{Medium Access Control} (MAC) sublayer of the \textit{Data Link Layer} (DLL) of the network stack explicitly handles this particular issue. When multiple nodes want to communicate at the same time, without any proper arrangement for the same, there can be repeated collision, which leads to a drastic drop in the network throughput, reliability, latency, and overall efficiency. Under traditional asynchronous transmission-based MAC strategies such as Aloha, CSMA/CA, CSMA/CD, etc., the nodes usually compete with each other to gain access to the medium. They waste a lot of bandwidth and energy in the nodes to mitigate the collisions among the packets from different nodes. %This strategy works quite well for small number of nodes and in single hop setup. However, the problem significantly scales up when the number of units grows and the mobile robotic units try to spread over more area. 

In contrast, under the \textit{concurrent transmission} paradigm, the nodes do not compete with each other. Instead, they cooperate in such a way that the RF packets emanating from different devices are transmitted exactly at the same time resulting in either \textit{capture effect} or \textit{constructive interference} in the physical layer of the network stack~\cite{rao2016murphy}. To realize this, the protocols depend on a strict \textbf{time synchronized transmission} and ensures that packets that are transmitted at the same time have exactly the same contents so that the signals instead of destroying each other \textit{interfere constructively} and results in a successful reception in the receiver.

Many fundamental communication problems are solved very efficiently using the concurrent transmission~\cite{jacob2019synchronous}. For example, one-to-all dissemination, i.e., network-wide flooding is achieved by Glossy \cite{ferrari2011efficient}, many-to-many data sharing and data aggregation are done by Chaos \cite{kaddoum2013design}, all-to-all and many-to-one communication are achieved by LWB \cite{sarkar2016lwb}, etc. It has been shown that these protocols can achieve reliability over 99.99\% under ultra-low radio power consumption and millisecond-level latency in communicating over 100s of nodes even in a multi-hop setup. Owing to such paramount capabilities, we propose to use concurrent transmission-based strategies for efficient multi-robot communication and collaboration. This point onward we refer to \textit{concurrent/synchronous transmission} by \textit{ST} and \textit{asynchronous transmission} by \textit{AT}.

In this work, we use an ST based protocol Glossy \cite{ferrari2011efficient} for a fast and energy-efficient one-to-all dissemination of information among mobile robots. The protocol fundamentally achieves the well-known network-wide flooding operation in a very energy and time-efficient manner. While traditional flooding protocol in a network of 100 nodes takes several minutes to converge, Glossy can achieve the same in a few 10s of milliseconds.

\subsection{Challenges in using ST in multi-robot-setting}
Although ST has various significant capabilities, there are certain fundamental problems in porting it to any generic multi-robot platform as well as its flexible inter-operation with other sub-systems \cite{amato2016policy}. ST based strategies need a precise sub-microsecond level time synchronization for effective simultaneous transmissions from different devices. The necessity to accomplish such a strict time synchronization, especially, under an infrastructure-less environment produces certain dependencies on the hardware. Simple fixed-length instruction based micro-controller architecture are more preferable for realizing such tight synchronization. The protocol Glossy exploits the events produced by the radio hardware during the packet reception and transmission coupled with appropriate adjustments in the CPU clock cycles in order to achieve the necessary time synchronization. It reuses the achieved synchronization to align the future packet transmissions and thereby maintaining the synchronization. However, precise clock-cycle level adjustments are hard to achieve in general micro-controller architecture. Although the inventor of Glossy provided a few directions on how to port it to any general hardware, so far, very few devices were shown to support successful multi-hop execution of this powerful protocol. Extremely tight coupling between external events (e.g., radio events) with the micro-controller operations happens to be a major bottleneck in using ST under a generic setting. In this work, we design a loosely coupled solution where ST is exploited despite the heterogeneity in the hardware.  %However, ST has been recently shown to be ported to some other radio technologies also in limited form such as BLE [YYY], Wideband [YYY: Ref] etc. But all these wirks have sho


%To accomplish a complex tasheik in a faster and efficient way, instead of a single robot, a swarm of simple robots can be used. Exploring unknown terrain in war field using a swarm of robo-cars [YYY], or underwater surveillance [YYY] by a swarm of robotic-fish [YYY], multi-drone application to build a 3D diagrams of an area, etc. are some common examples applications of such swarm robots. 
%The \textit{Network Stack}, inside the OS (as shown in the Figure \ref{YYY}(a)), is in charge of the communication with other robots. The MRC applications uses the facilities to achieve an effective collaboration among multiple robots. However, poor scalability, poor energy efficiency, high latency, etc., are some of major drawbacks in the M
%Its well known that RF communication consumes more power from the battery and hence assumption of long range communication facilities with the power constraints robots cannot be a realistic assumption. Thus, the robots need to depend on multi-hop communication where each robot has limited communication range and hence, a message from one robot is conveyed to to the destination robot through one or more robots in between. However, due to lack of global view of the neighborhood in any of the robots, such multi-hop communication brings many other challenges [Ref:some chaotic]. Even a simple communication task such as disseminating a single piece of information to all the robots may create huge number of redundant messages wasting a lot of battery power as well as spend of a lot of time unnecessarily. To handle its complexity the task the networks functionalities are divided in multiple layers. Under the standard TCP/IP protocol suit, the network layer in figure \ref...(a) itself is divided in 5 sub-layers \textit{Physical Layer, Data Link Layer, Network Layer(IP), Transport Layer (TCP) and Application Layer}. (b). 




==> 4-implementation.tex <==
% \subsection{State diagram} \label{sec:implementation}

% The state diagram of the overall system comprising of CCU and NU is given in Fig.~\ref{fig:state-diagram}. The two components are governed by different state machines. The right side of the figure shows the state diagram of NU running the Glossy protocol while the left side shows the state diagram of the CCUs, which in our case, run the PID controllers. In our work to keep the application simple, we consider a leader-follower framework where a single leader device always tries to inform its current wheel speed value to all the follower devices. The followers try to dynamically adjust their speed as per the received speed from the leader. In the case of Glossy protocol, we have only one initiator, and hence we let the leader device be the Glossy initiator also. And the 2 fat arrows flowing between the components in the state diagram represent the data flow through the Serial Line Protocol (SLP). Through this split architecture, the followers receive the leader's status and along with their current status, they try to adjust their wheel speeds. On the other hand, the leader periodically reads its current status, updates it as per its target, and transmits the status to the followers through the Glossy protocol.

\begin{figure*}[t!]
\begin{center}
\includegraphics[width=0.9\linewidth]{Figures/loop_6.pdf}
\end{center}
\caption{State diagram.} \label{fig:state-diagram}
\end{figure*}


The period of the Glossy protocol running in the NUs in a loop is referred to as \textit{Glossy Period} (GP). Similarly, the PID controller governing the behavior of the robotic systems also run a loop for periodic correction of the errors, i.e., the deviations from the reference speed. This is referred to as \textit{PID-loop} and the period of the same is referred to as \textit{PID-period} or PP. % After the NU-NU communication part in the GP, the followers receive the state information of the leader. Similarly, before the beginning of the packet NU-NU communication part the leader reads its own state information and prepares the packet to be communicated to the corresponding NU. 
In general GP and PP can take a wide range of values. In case of a lower value of PP, the robot can more dynamically adapt to changes in the status. But too low a value of PP may result in insufficient error accumulation especially in case of large changes. Similarly, a higher value of PP may also result in the inability of the device to adapt to more frequent changes as per requirements. In the case of GP, the higher the period value, the lesser the duty cycle of the radio. However, due to internal clock drift, too large value of the GP period may bring trouble to the base synchronization. Fig.~\ref{fig:loops} shows a possible pattern of interaction between GP and PP. The vertical arrows indicate the dissemination of the leader's information at different GP period while the horizontal arrow shows a possible time lag between the point of time where the leader's information is received and the point in time when it is going to be considered for further action in the follower. Thus, an important aspect of fruitful use of the ST strategies for a multi-robotic system is to decide the correct combination of the duration of PP and GP. In general for any given sequence of changes, the Follower PP (FPP) should be at least as small as Leader PP (LPP)so that the follower can change the status as fast as the leader. A lower LPP period is not necessary and a higher LPP period may result in inappropriate following by the followers. %However, note that the GP period should be at least as low as the SP duration for follower so that follower does not receive a new change request in between stabilization of the previous period. Even if the GP is lower than that, the values are required to be ignored.
A significant part of our evaluation study deals with understanding the relationship between the GP as well as FPP and LPP.

%We consider the implementation of a simple MRC application where the devices will try to follow a set of instructions synchronously which necessary local changes. From that sense an unit may behave as a leader from where the commands will originate or it may work as a follower ...
%where one device acts as a leader a set of nodes will try to execute some commands originating from either i one device will disseminate its current state - the flooding algorithm which we use for disseminating the information from leader to all the followers. 
%Almost every ST based protocol runs in iterations. Its equivalent to loop where the starting part of the loop very small amount of time the actual fast and compact communication takes places while the rest of the loop remains free of any radio-usage. The structure is present in Chaos, and many other ST based protocols. 

%Note that, once the reference value is set, the effect does not takes place instantaneously in the implementing PID controller. It takes some time to stabilize to the necessary status. This stabilization time varies with reference points. We call this as SP.


% \begin{figure}[t!]
% \begin{center}
% \includegraphics[width=\textwidth]{Figures/two-loops.pdf}
% \end{center}
% \caption{Interaction between PID loop and Glossy loop.} \label{fig:loops}
% \end{figure}


==> 7-relatedworks.tex <==
\section{related works}\label{sec:relatedwork}
In coordinated control, a group of autonomous robots follows predefined trajectories while maintaining the desired spatial pattern, which is called formation control. In formation control, different control topologies and approaches can be adopted depending on the specific scenarios, for example, leader-follower strategy \cite{li2016affection, lin2020adaptive}, virtual structure approach \cite{nazari2016decentralized, wu2020decentralized} and behavior-based method \cite{balch1998behavior, yu2019formation}. Teams of coordinated robot control has several unique advantages over single robot across many domains of task such as precision agriculture \cite{barrientos2011aerial, kazmi2011adaptive}, logistics \cite{farinelli2017advanced}, rescue operations \cite{kantor2003distributed, liu2016multirobot} and mapping \cite{howard2006multi}, etc. However, there are several challenges in designing effective multi-robot systems, such as the high dimensionality of a team that makes planning and decision-making a difficult task. To support those decisions in a realistic setting by communicating information across the team makes it even more difficult. As a result, in a real environment, it requires a central authority to control effective unrestricted communication, which may lead to hard solutions or limited scalability. 

%In this paper, our focus is on the leader follower control, in which one or more robots can be leaders in the group while other robots follow one or more leaders in a specified topological way. Multi-robot formation control based on leader-follower scheme performed by team of mobile robots forming a specific shape requires specific algorithms, strategies and controllers to control robots in longitudinal and lateral direction. More importantly, multi-robot formation control highly depend on the ability to exchange information among each other's over a network of communication systems that is steady, continuous or intermittent. In an ideal situation, every robots should be able to communicate with each other, exchange information and should be aware of their position with respect to each other. Therefore, the information sharing plays a vital role to achieve overall goal of formation control. However, it would be very expensive process to have all the global information available to each robot. To have a cost effective formation, the followers should at least continuously or intermittently know the position of themselves with regard to leader. 

Several works exist in the literature on different communication protocols and control strategies for leader-follower formation control \cite{kanayama1990stable, abdessameud2016leader}. However, most of the works are based on the theoretical studies \cite{pereira2003formation, chen2011leader, loria2015leader, panagou2014cooperative} or implemented various protocols/algorithms in simulation platforms \cite{chehardoli2018third, maghenem2018robust}. A very few works are done in practical setups \cite{wurman2008coordinating, widyotriatmo2017implementation}. But those were not yet at the level of commercialization due to the lack of communication speed and proper control strategies. Hence, there is still require a lot of effort to establish better communication protocols and control strategies to achieve leader-follower formation control.  

Loria \textit{et al.}~\cite{loria2015leader} presented an implementation of the communication topology that forms a simple directed spanning-tree for a leader-follower formation control approach, assuming that only one swarm leader robot has the information of the reference trajectory and each follower robot receives information from one intermediary leader only. The advantage of this communication protocol is the simplicity of its implementation, e.g., fewer sensors are needed. Alternatively, Dimarogonas \textit{et al.}~\cite{dimarogonas2007rendezvous} proposed a decentralized feedback control strategy for multiple mobile robots that forms an undirected communication graph that represents the inter-robot communication topology. The authors recommended working on switching communication topologies to measure the performance of the formation-tracking controller. Wan \textit{et al.}~\cite{wan2017semi} employed a leader-follower semi-centralized approach to form the formation of the robots using the Hungarian method. 
%In the first phase, robots selected a leader and move by following the leader. Next, robots establish a formation with respect to a center such as the center of a square, circle, and triangle. 
In another work, a decentralized leader-follower tracking-agreement controller was proposed that used relative velocity and position measurement of the robot with respect to a leader robot \cite{maghenem2018robust}. According to this communication topology, the consensus is achieved if it holds for each and all possible open chains, subsets of the spanning tree. They assume that there exists an open-chain composed of all robots, each having one follower and one leader. To illustrate the results, they only performed simulation tests. %and didn't conduct experiments with real robots. 
Abdessameud \textit{et al.}~\cite{abdessameud2016leader} addresses the leader-follower synchronization problem of uncertain networked Euler-Lagrange systems under directed interconnection graphs in the presence of communication constraints using an adaptive distributed control algorithm such that a group of Euler-Lagrange systems asymptotically synchronize their states to those of a dynamic leader with a time-varying trajectory. 
%The information exchange between all systems in the network is through a directed interconnected graph containing a spanning tree. 
However, the communication is assumed to be discrete in time, intermittent, and subject to irregular communication delays and possible packets dropouts. They have validated the effectiveness of the proposed control scheme using simulation and not on real robots.

In a parallel approach, researchers used a vision-based formation control strategy without using any communication protocol \cite{mariottini2009vision, li2018neural}. For example, an active vision algorithm was proposed by Chen \textit{et al.}~\cite{chen2015adaptive} to achieve adaptive leader-follower formation control in the absence of communication. Instead, a follower robot tracks the features of a leader robot through a camera by providing visual measurements and a formation controller to maintain formation. In \cite{vision-based-formation}, a vision-based cooperative formation control method has been proposed. The experimental system consists of a UAV (Unmanned Aerial Vehicle) and multiple UGVs (Unmanned Ground Vehicles). 
%The authors aim at controlling the multi-UGVs to the desired formation relying only on the visual information obtained by a camera mounted on the UAV. 
The work in \cite{limited-sensor-view} focuses on the problem of quadrotor formation control. The issue of the limited sensor field of view has been addressed. The proposed solution enables the quadrotors to take their right positions in the desired formation, even when the sensor view is restricted. Furthermore, a vision-based leader-follower formation control was achieved by developing a neural-dynamic optimization-based nonlinear model predictive control \cite{li2018neural}. In this study, a camera on the follower robot was employed to track the features and to measure the state and velocity of the leader robot. However, there is a limitation with vision-based formation control as the sensor has a limited range of visibility. It is inconvenient to apply a vision-based system for a broad range of applications without any proper communication protocol. 



%In this paper, we have proposed a synchronous communication protocol for multi-robot leader-follower formation control scheme, which may overcome the drawbacks of other existing communication protocols. A  synchronous transmission based fast and energy-efficient communication framework is proposed that can be scalable upto 100's or 1000's of robots having various types of hardware platforms. We demonstrate the effectiveness of the proposed strategy by performing several experiments with a group of five robots, where one is act like a leader and others are considered as followers. The robots successfully form a desired circle, rectangle, triangle shape of formation with the proposed communication protocol and control strategies.  

 
%The work \cite{2011-multirobot-rectangle} shows an implementation ....

%In \cite{self-organizing-formation}, the authors propose a self-organizing approach for both circle and polygon formation for multiple unmanned aerial vehicles (MUAV-s). Where existing works usually require that UAVs have unlimited sensing and communication range, the proposed solution removes this assumption. The UAV-s considered are capable of localization,communication and sensing. Each UAV communicates with neighbours that lie within its communication range.

%\cite{distributed-formation-control} presents a distributed method for navigating a team of robots in formation in 2D and 3D environments with static and dynamic obstacles. The robots are assumed to have a reduced communication and visibility radius and share information with their neighbors. Formation control is achieved by means of distributed consensus.



%Summarize the following 
%https://www.seas.upenn.edu/~jadbabai/papers/$2006ACC_1465_FI.pdf$

%http://techlav.ncat.edu/publications/Formation%20Control.pdf

%This is new domain - where we should focus - our work is a way towards solving the problem using synchronous transm
%https://ieeexplore.ieee.org/abstract/document/5313866

%Next go to the papers that are citing these papers - check which papers are relevant to us and summarize some of them here.

%\textit{At least one agent plays a role as aleader and the rest of the agents are designated as followers. The followers track the position of the leader with some prescribed offsets while the leader tracks its desired trajectory}. Check with Sudipta. 
  
%In \cite{do2007nonlinear} author employed a combination of the virtual structure and path-tracking approaches to generate the reference for each robots under the assumption that the translational leader velocity is persistently exciting. Several controllers were developed for the formation control of the multiple vehicles targeting a leader–follower tracking problem such as feedback linearization controller for formation maintenance, an adaptive controller to achieve ideal control due to inaccurate relative distance and a robust adaptive controller to cope with the external interference \cite{li2017multiple}.

%The advantage of this approach is the reduced tracking errors and can be analysed using standard control techniques \cite{chunyu2009new}. 

%Another benefit is that only the leader is responsible for planning trajectories and followers must follow the coordinates of the leader; therefore, it results in a simple controller. In terms of disadvantage, a leader’s fault can penalise the whole formation and feedback from followers to a leader is generally not applied in this approach.
  
%In the leader-follower approach, a leader is assigned to the multi-robot formation and remaining robots are the followers. In this approach, a leader follows its desired trajectory while follower robots track the position of the leader. There are three kinds of leader in this approach, namely static leader, dynamic leader and virtual leader. 

